On Grounded Planning for Embodied Tasks with Language Models

Language models (LMs) have demonstrated their capability in possessing commonsense knowledge of the physical world, a crucial aspect of performing tasks in everyday life. However, it remains unclear **whether LMs have the capacity to generate grounded, executable plans for embodied tasks.** This is a challenging task as LMs lack the ability to perceive the environment through vision and feedback from the physical environment. In this paper, we address this important research question and present the first investigation into the topic. Our novel problem formulation, named **G-PlanET**, inputs a high-level goal and a data table about objects in a specific environment, and then outputs a step-by-step actionable plan for a robotic agent to follow. To facilitate the study, we establish an **evaluation protocol** and design a dedicated metric to assess the quality of the plans. Our experiments demonstrate that the use of tables for encoding the environment and an iterative decoding strategy can significantly enhance the LMs' ability in grounded planning. Our analysis also reveals interesting and non-trivial findings.

==> 9_limitations.tex <==
The main limitations of this work on the new task~\taskname{} are as follows:
\begin{itemize}
    \item \textbf{Evaluation}: Although we have adopted and devised automatic metrics for evaluating methods for~\taskname{}, there is not yet a straightforward way for us to test the ultimate success rates of such plans (if they were executed by oracle agents). We tried using state-of-the-art ALFRED agents such as FILM~\cite{Min2021FILMFI}, but they did not show obvious differences using step-by-step instructions (even if using the oracle version). We believe more human evaluation will help us further refine the metrics, which can be very expensive though. It is because human annotators much play with the 3D engine while following these instructions, in order to assess the quality of such plans. 
    \item \textbf{Methods:} Flattening object tables into sequences of tokens row by row is straightforward but might not be optimal. The number of objects can be huge for a complicated room. How can we narrow down the important objects at each step? We argue that a more advanced version of attention modules for dynamic table encoding is needed. We may not need to input the whole table for decoding at all steps. As a preliminary study, we created a retrieval augmentation method that only includes the oracle objects (that are mentioned in the next step) as the input, but we see little improvement. We think more physical rules and math computation with the object features will help us gain more improvement. 
\end{itemize}

% The number of objects that are actually relevant to task completion is limited compared to the objects within the entire environment. Is there some way to filter out relevant objects to improve the success rate of model planning? We are also very excited to see the results of model-generated plans compared to human handwritten ones during real interactions, which may be called agent-based evaluation. We tried this work on FILM and did not get significant results. We expect that there will be subsequent work using low-level instruction to help us verify the ability of the model on grounded planning. It is also expected that a model architecture or pipeline for this task will be proposed.

==> figure/reweight_spice.tex <==
% \begin{figure}[t!]
% \centering
% \begin{tikzpicture}
% \small{
% \begin{axis}[
% at={(0,0)},
% width=.4\textwidth, height=.35\textwidth ,
% xtick={0, 1, ..., 10},
% xticklabels={
%  {$0$}, {$ $}, {$0.2$}, {$ $}, {$0.4$},
%  {$ $}, {$0.6$}, {$ $}, {$0.8$}, {$ $},{$1$}
% },
% ytick={0.20,0.25,...,0.60},
% yticklabels={{$0.20$}, {$0.25$}, {$0.30$}, {$0.35$}, {$0.40$}, {$0.45$}, {$0.50$}, {$0.55$}, {$0.60$}},
% grid style=dashed,
% ylabel={Performance},
% xlabel={{P}},
% xlabel style={yshift=0.5em},
% ylabel style={align=center,yshift=-1em},
% y tick style={opacity=0},
% ymajorgrids=true,
% xmajorgrids=true,
% tick align=inside,
% legend pos=outer north east,
% yticklabel style={/pgf/number format/precision=1,/pgf/number format/fixed zerofill},
% legend style={yshift=0em,xshift=-6.8em,legend cell align=left,legend plot pos=right},
% xmin=-0.5,
% xmax=10,
% ymin=0.20,
% ymax=0.60]
%     \addplot[
%         red!60,mark=pentagon*,mark size=1.7pt,thick,line width=1pt,mark options={fill=white,draw=red,line width=0.5pt}
%         ]
%         coordinates {
%         (0, 0.31684431192253737)
%         (1, 0.31127295864973853)
%         (2, 0.30730654717179157)
%         (3, 0.3036738615393242)
%         (4, 0.2992416867239351)
%         (5, 0.29335238882439907)
%         (6, 0.28573847389556084)
%         (7, 0.276303063943734)
%         (8, 0.26493372311589475)
%         (9, 0.25140080465709486)
%         (10, 0.23534790678798137)
%         };
%       \addplot[
%         blue!60,mark=square*,mark size=1.2pt,thick,line width=1pt,mark options={fill=white,draw=blue,line width=0.5pt}
%         ]
%         coordinates {
%         (0, 0.34905618386844584)
%         (1, 0.3423302540918126)
%         (2, 0.3372216737116396)
%         (3, 0.3325517586078169)
%         (4, 0.32726427661208213)
%         (5, 0.3207197555083438)
%         (6, 0.3126351596203602)
%         (7, 0.3029063009038285)
%         (8, 0.2914268381611666)
%         (9, 0.27796327133939286)
%         (10, 0.26211806289943684)
%         };
%         \addplot[
%         magenta!80,mark=triangle*,mark size=1.9pt,thick,line width=1pt,mark options={fill=white,draw=magenta,line width=0.5pt}
%         ]
%         coordinates {
%         (0, 0.5054096131035745)
%         (1, 0.48080073713441834)
%         (2, 0.45481013789425156)
%         (3, 0.4280658395134587)
%         (4, 0.4014278522284052)
%         (5, 0.37557793578532606)
%         (6, 0.3508742223154198)
%         (7, 0.32736594736113894)
%         (8, 0.30480453756203135)
%         (9, 0.28262567814911094)
%         (10, 0.2599375470221303)
%         };
%         \addplot[
%         cyan!80,mark=square*,mark size=1.2pt,line width=1.2pt,mark options={fill=white,draw=cyan,line width=0.5pt,solid}
%         ]
%         coordinates {
%         (0, 0.5194285728933805)
%         (1, 0.48814104642248246)
%         (2, 0.45736405379712336)
%         (3, 0.4277606630293626)
%         (4, 0.39956854815980386)
%         (5, 0.372778992163757)
%         (6, 0.34728492801556404)
%         (7, 0.3228919286213619)
%         (8, 0.2992559726595239)
%         (9, 0.27580931950553117)
%         (10, 0.2517162978194509)
%         };
%         \addplot[
%         pink!60,mark=triangle*,mark size=1.9pt,mark options={fill=white,draw=pink,line width=0.5pt,solid},line width=1pt
%         ]
%         coordinates {
%         (0, 0.5209648071334182)
%         (1, 0.4921390463810853)
%         (2, 0.46371599953965337)
%         (3, 0.43621823556382405)
%         (4, 0.409859013588879)
%         (5, 0.3846932195206426)
%         (6, 0.3606862708289208)
%         (7, 0.3376979006340092)
%         (8, 0.315422690537387)
%         (9, 0.2933169355692448)
%         (10, 0.2705489197507247)
%         };
%         \legend{\tiny{Vanilla},\tiny{Table},\tiny{\textsc{TaPEx}},\tiny{Table Iter},\tiny{\textsc{TaPEx} Iter}}
% \end{axis}
% }
% \end{tikzpicture}
% \caption{The step-wise reweighting results of SPICE.}
% \label{fig5}
% \end{figure}
